Enhancing Tool Calling in LLMs with the International Tool Calling Dataset

Tool calling allows large language models (LLMs) to interact with external systems like APIs, enabling applications in customer support, data analysis, and dynamic content generation. While recent benchmarks have advanced tool-use research, they suffer from key limitations, including reliance on simulated or restricted APIs, limited reproducibility, and a lack of cultural and geographic diversity. To address these gaps, we introduce International Tool Calling (ITC), a large-scale, multilingual benchmark designed for realistic, globally distributed tool-calling scenarios. ITC includes 3,571 real APIs and 17,540 tool calling tasks across 20 categories and 40 countries. Experiments reveal substantial performance gaps between open- and closed-source LLMs, while fine-tuning on ITC yields significant improvements, particularly for non-English queries, enhancing cross-lingual generalization, reasoning consistency, and robustness to out-of-domain tools. ITC provides a valuable benchmark for advancing LLM robustness and performance in complex, multi-tool, and international scenarios. Dataset: https://anonymous.4open.science/r/International-Tool-Calling-ITC-dataset-FAF4/.

==> text/Dataset_Maintenance_and_Sustainability.tex <==
% 回答审稿人 6zzm的问题：The reliance on free, public APIs means that the dataset is inherently unstable—API endpoints, parameters, and outputs may change or disappear over time. This undermines the reproducibility of the benchmark and the long-term value of the dataset, especially since the main contribution is the dataset itself. The paper acknowledges this limitation but does not propose concrete solutions or mitigation strategies.
We acknowledge the valid concern regarding the inherent instability of using free, public APIs, which could impact the long-term value and reproducibility of our benchmark. To address this proactively, we have established a comprehensive maintenance and mitigation strategy to ensure the sustainability of the ITC dataset.

We are developing an automated monitoring pipeline to periodically (e.g., monthly) test all API endpoints in the dataset for availability, authentication, and schema consistency. The results will be published on a \textbf{publicly accessible health dashboard} linked from our dataset repository. This transparency allows researchers to track the real-time status of each API and filter for the most reliable ones in their experiments.

The ITC dataset is hosted on GitHub to foster community involvement. We encourage users to report broken APIs via issues and contribute new tools or updates via pull requests. This community-driven approach will help maintain the dataset's quality and relevance over time, making it a sustainable and evolving resource.

